Optimal Taxes in Atomic Congestion Games

How can we design mechanisms to promote efficient use of shared resources? Here, we answer this question in relation to the well-studied class of atomic congestion games, used to model a variety of problems, including traffic routing. Within this context, a methodology for designing tolling mechanisms that minimize the system inefficiency (price of anarchy) exploiting solely local information is so far missing in spite of the scientific interest. In this manuscript we resolve this problem through a tractable linear programming formulation that applies to and beyond polynomial congestion games. When specializing our approach to the polynomial case, we obtain tight values for the optimal price of anarchy and corresponding tolls, uncovering an unexpected link with load balancing games. We also derive optimal tolling mechanisms that are constant with the congestion level, generalizing the results of Caragiannis et al. [ACM Transactions on Algorithms, 2010] to polynomial congestion games and beyond. Finally, we apply our techniques to compute the efficiency of the marginal cost mechanism. Surprisingly, optimal tolling mechanism using only local information perform closely to existing mechanism that utilize global information [Bil\`o and Vinci, ACM Transactions on Economics and Computation, 2019], while the marginal cost mechanism, known to be optimal in the continuous-flow model, has lower efficiency than that encountered levying no toll. All results are tight for pure Nash equilibria, and extend to coarse correlated equilibria.

==> Tex final - to submit ArXiv/figures-tex/figure-regions.tex <==
\begin{figure}[h!]
\begin{center}
\begin{tikzpicture}[scale=1]
\draw[thick,->] (0,0) -- (3,0);
\draw[thick] (3.2,-0.1) -- (3.2,-0.1) node[anchor=north east]{$\u$};
\draw[thick,->] (0,0) -- (0,3); 
\draw[thick] (0,3.2) -- (0,3.2) node[anchor=north east]{$\v$};
\draw[-] (2,0) -- (2,2) ;
\draw[-] (0,2) -- (2,2) ;
\draw[dashed] (0,2) -- (1,1) ;
\draw[dashed] (1,1) -- (1,2) ;
\draw[dashed] (1,1) -- (2,0) ;
\draw[dashed] (0,0) -- (2,2) ;
\node[rotate = 45] at (0.7,0.5) {\small$\v=\u$};
\node at (0.4,1) {\small A};
\node at (0.7,1.7) {\small B};
\node at (1.3,1.7) {\small C};
\draw[thick] (0,0.1) -- (0,-0.1) node[anchor=north]{\footnotesize$0$};
\draw[thick] (0.5,0.1) -- (0.5,-0.1)node[anchor=north]{\footnotesize$1$};
\draw[thick] (2,0.1) -- (2,-0.1);
\draw[thick] (2,-0.1) -- (2,-0.1)node[anchor=north]{\footnotesize$n$};
\node[thick] (a) at (1.25,-0.3) {$\dots$};
\draw[thick] (0.1,0) -- (-0.1,0)node[anchor=east]{\footnotesize$0$};
\draw[thick] (0.1,0.5) -- (-0.1,0.5)node[anchor=east]{\footnotesize$1$};
\node[thick] (a) at (-0.3,1.25) {$\vdots$};
\draw[thick] (0.1,2) -- (-0.1,2)node[anchor=east]{\footnotesize$n$};
\end{tikzpicture}
\vspace*{-2mm}
\end{center}
\caption{Regions A, B, and C utilized in proof of \cref{lem:v>u_does_not_matter}.\vspace*{-2mm}}
\label{fig:figure2proof}
\end{figure}

==> Tex final - to submit ArXiv/figures-tex/figure3.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}
\newlength{\myedgewidth}
\setlength{\myedgewidth}{0.8pt}
  \Vertex[x=1.4, y=0.8,  color=pnasblueback, label={\large$\rm{O}_1$}, style={line width=\myedgewidth}]{C}
  \Vertex[x=1.4, y=-0.8,  color=pnasblueback, label={\large$\rm{O}_2$}, style={line width=\myedgewidth}]{D}
  \Vertex[x=1, y=0,  color=pnasblueback, size=0.2, style={line width=\myedgewidth}]{betweenCDleft}
  \Vertex[x=1.8, y=0,  color=pnasblueback, size=0.2, style={line width=\myedgewidth}]{betweenCDright}
  \Vertex[x=3, y=0,  color=pnasblueback, label={\large\rm{D}}, style={line width=\myedgewidth}]{E}
  \Edge[Direct, bend=-15, lw=\myedgewidth, color=black](C)(betweenCDleft)
  \Edge[Direct, bend=-15, lw=\myedgewidth, color=black](betweenCDright)(C)
  \Edge[Direct, bend=-15, lw=\myedgewidth, color=black](betweenCDleft)(D)
  \Edge[Direct, bend=-15, lw=\myedgewidth, color=black](D)(betweenCDright)
  \Edge[Direct, lw=\myedgewidth, color=black](C)(E)
  \Edge[Direct, lw=\myedgewidth, color=black](D)(E)
  \Text[x=2.2, y=0.8, fontsize=\small]{$x$}
  \Text[x=2.2, y=-0.8, fontsize=\small]{$x$}
  \Text[x=0.95, y=0.4, fontsize=\small]{$x$}
  \Text[x=1.85, y=0.4, fontsize=\small]{$x$}
  \Text[x=0.95, y=-0.4, fontsize=\small]{$x$}
  \Text[x=1.85, y=-0.4, fontsize=\small]{$x$}
  \Text[x=1.5, y=-1.6, fontsize=\footnotesize]{Nash routing, $\tau_e(x)=0$}
  \Text[x=1.52, y=-2, fontsize=\footnotesize]{(A)~~System Cost: 2}%
  \Vertex[x=1.34, y=1, Pseudo, size=0]{N2bid}
  \Vertex[x=3, y=0.15, Pseudo]{N3}
  \Edge[color=red, Direct](N2bid)(N3)
  \Vertex[x=1.34, y=-1, Pseudo, size=0]{bisN2bid}
  \Vertex[x=3, y=-0.15, Pseudo]{bisN3}
  \Edge[color=blue, Direct, style={dashed}](bisN2bid)(bisN3)  
\end{tikzpicture}
\hspace*{10mm}
\begin{tikzpicture}
\setlength{\myedgewidth}{0.8pt}
  \Vertex[x=1.4, y=0.8,  color=pnasblueback, label={\large$\rm{O}_1$}, style={line width=\myedgewidth}]{C}
  \Vertex[x=1.4, y=-0.8,  color=pnasblueback, label={\large$\rm{O}_2$}, style={line width=\myedgewidth}]{D}
  \Vertex[x=1, y=0,  color=pnasblueback, size=0.2, style={line width=\myedgewidth}]{betweenCDleft}
  \Vertex[x=1.8, y=0,  color=pnasblueback, size=0.2, style={line width=\myedgewidth}]{betweenCDright}
  \Vertex[x=3, y=0,  color=pnasblueback, label={\large\rm{D}}, style={line width=\myedgewidth}]{E}
  \Edge[Direct, bend=-15, lw=\myedgewidth, color=black](C)(betweenCDleft)
  \Edge[Direct, bend=-15, lw=\myedgewidth, color=black](betweenCDright)(C)
  \Edge[Direct, bend=-15, lw=\myedgewidth, color=black](betweenCDleft)(D)
  \Edge[Direct, bend=-15, lw=\myedgewidth, color=black](D)(betweenCDright)
  \Edge[Direct, lw=\myedgewidth, color=black](C)(E)
  \Edge[Direct, lw=\myedgewidth, color=black](D)(E)
  \Text[x=2.2, y=0.8, fontsize=\small]{$x$}
  \Text[x=2.2, y=-0.8, fontsize=\small]{$x$}
  \Text[x=0.95, y=0.4, fontsize=\small]{$x$}
  \Text[x=1.85, y=0.4, fontsize=\small]{$x$}
  \Text[x=0.95, y=-0.4, fontsize=\small]{$x$}
  \Text[x=1.85, y=-0.4, fontsize=\small]{$x$}
  \Text[x=1.5, y=-1.6, fontsize=\footnotesize]{Nash routing, $\pig{\tau}_e(x)=x-1$}
  \Text[x=1.5, y=-2, fontsize=\footnotesize]{(B)~~System cost: 6}
  \Vertex[x=1.34, y=1, Pseudo, size=0]{N2bid}
  \Vertex[x=3, y=0.15, Pseudo]{N3}
  \Vertex[x=1.22, y=0.85, Pseudo]{N4}
  \Vertex[x=1.22, y=-0.85, Pseudo]{N5}
  \Edge[color=blue, Direct, style={dashed}](N2bid)(N3)
  \Edge[color=blue, style={dashed}, bend=-40](N5)(N4)
  \Vertex[x=1.34, y=-1, Pseudo, size=0]{bisN2bid}
  \Vertex[x=3, y=-0.15, Pseudo]{bisN3}
  \Vertex[x=1.58, y=-0.85, Pseudo]{bisN4}
  \Vertex[x=1.58, y=0.85, Pseudo]{bisN5}
  \Edge[color=red, Direct](bisN2bid)(bisN3)
  \Edge[color=red, bend=-40](bisN5)(bisN4)
\end{tikzpicture}
\vspace*{-2mm}
\caption{
Instance used to demonstrates that the price of anarchy associated to the marginal cost toll mechanism is at least $3$ in affine congestion games. Two users are willing to travel from $\rm{O}_1/\rm{O}_2$ to $\rm{D}$, where each edge features a cost $\ell_e(x)=x$. In the un-tolled case (A) the system cost at the worst Nash-equilibrium is $2$. The situation worsens when using marginal cost tolls (B), as the worst Nash equilibrium gives a system cost of $6$.}
\vspace*{-2mm}
\label{example:tolledpigouvian}
\end{figure}


==> Tex final - to submit ArXiv/figures-tex/figureBF1.tex <==
\newcommand\radius{2.4}
\begin{figure}[b!]
\begin{center}
\hspace*{-5mm}
\raisebox{-0.55\height}{\begin{tikzpicture}[scale=0.45, transform shape]%
\begin{scope}
\clip (0,0)-- +(90:\radius + 2) arc (90:225-360:\radius + 2) -- cycle;
\draw[red,thick,fill=red,fill opacity=0.2] (0,0) circle (\radius + 0.75);
\draw[red,thick,fill=white] (0,0) circle (\radius - 0.75);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(90:\radius + 2) arc (90:135:\radius + 2) -- cycle;
\draw[red,thick,fill=red,fill opacity=0.2] (\fpeval{\radius*cos(90*pi/180)},\fpeval{\radius*sin(90*pi/180)}) circle(0.75);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(225:\radius + 2) arc (225:180:\radius + 2) -- cycle;
\draw[red,thick,fill=red,fill opacity=0.2] (\fpeval{\radius*cos(225*pi/180)},\fpeval{\radius*sin(225*pi/180)}) circle(0.75);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(180:\radius + 2) arc (180:135:\radius + 2) -- cycle;
\draw[blue,thick,fill=blue,fill opacity=0.2] (0,0) circle (\radius + 0.75);
\draw[blue,thick,fill=white] (0,0) circle (\radius - 0.75);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(180:\radius + 2) arc (180:225:\radius + 2) -- cycle;
\draw[blue,thick,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(180*pi/180)},\fpeval{\radius*sin(180*pi/180)}) circle(0.75);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(135:\radius + 2) arc (135:90:\radius + 2) -- cycle;
\draw[blue,thick,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(135*pi/180)},\fpeval{\radius*sin(135*pi/180)}) circle(0.75);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(45:\radius + 2) arc (45:180-360:\radius + 2) -- cycle;
\draw[red,thick,dashed,fill=red,fill opacity=0.2] (0,0) circle (\radius + 0.9);
\draw[red,thick,dashed,fill=white] (0,0) circle (\radius - 0.9);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(45:\radius + 2) arc (45:90:\radius + 2) -- cycle;
\draw[red,thick,dashed,fill=red,fill opacity=0.2] (\fpeval{\radius*cos(45*pi/180)},\fpeval{\radius*sin(45*pi/180)}) circle(0.9);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(180:\radius + 2) arc (180:135:\radius + 2) -- cycle;
\draw[red,thick,dashed,fill=red,fill opacity=0.2] (\fpeval{\radius*cos(180*pi/180)},\fpeval{\radius*sin(180*pi/180)}) circle(0.9);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(135:\radius + 2) arc (135:90:\radius + 2) -- cycle;
\draw[blue,thick,dashed,fill=blue,fill opacity=0.2] (0,0) circle (\radius + 0.9);
\draw[blue,thick,dashed,fill=white] (0,0) circle (\radius - 0.9);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(135:\radius + 2) arc (135:180:\radius + 2) -- cycle;
\draw[blue,thick,dashed,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(135*pi/180)},\fpeval{\radius*sin(135*pi/180)}) circle(0.9);
\end{scope}%
\begin{scope}
\clip (0,0)-- +(90:\radius + 2) arc (90:45:\radius + 2) -- cycle;
\draw[blue,thick,dashed,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(90*pi/180)},\fpeval{\radius*sin(90*pi/180)}) circle(0.9);
\end{scope}%
\fill[fill = white] (0,0) circle (\radius - 0.91);%
\foreach \n in {0,1,2,3,4,5,6,7}{
	\draw (\fpeval{\radius*cos(\n*pi/4)},\fpeval{\radius*sin(\n*pi/4)}) node[circle,draw]{$\mygamma/8$};}%
\node[red] at (\fpeval{(\radius+1.25)*cos(3*pi/8)},\fpeval{(\radius+1.25)*sin(3*pi/8)}) {\Huge$\NE{a}_1$};%
\node[blue] at (\fpeval{(\radius+1.25)*cos(7*pi/8)},\fpeval{(\radius+1.25)*sin(7*pi/8)}) {\Huge$\opt{a}_1~$};%
\node[red] at (\fpeval{(\radius+1.5)*cos(1*pi/8)},\fpeval{(\radius+1.5)*sin(1*pi/8)}) {\Huge$\NE{a}_2$};%
\node[blue] at (\fpeval{(\radius+1.5)*cos(5*pi/8)},\fpeval{(\radius+1.5)*sin(5*pi/8)}) {\Huge$\opt{a}_2$};%
\end{tikzpicture}}%%
\hspace*{-5mm}
\raisebox{-0.5\height}{
\begin{tikzpicture}[scale=0.45, transform shape]
\draw[blue,thick,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(180*pi/180)},\fpeval{\radius*sin(180*pi/180)}) circle(0.75);
\draw[blue,thick,dashed,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(135*pi/180)},\fpeval{\radius*sin(135*pi/180)}) circle(0.9);
%
\foreach \n in {0,1,2,3,4,5,6,7}{
	\draw (\fpeval{\radius*cos(\n*pi/4)},\fpeval{\radius*sin(\n*pi/4)}) node[circle,draw]{$\mybeta/8$};}
\node[blue] at (\fpeval{(\radius+1.25)*cos(8*pi/8)},\fpeval{(\radius+1.25)*sin(8*pi/8)}) {\Huge$\opt{a}_1~$};
%
\node[blue] at (\fpeval{(\radius+1.5)*cos(6*pi/8)},\fpeval{(\radius+1.5)*sin(6*pi/8)}) {\Huge$\opt{a}_2$};
\end{tikzpicture}}
\hspace*{2mm}
\raisebox{-0.5\height}{
\begin{tikzpicture}
\draw (0,-2.2) -- (0,1.7);	
\end{tikzpicture}}
\hspace*{-7mm}
\raisebox{-0.5\height}{
\begin{tikzpicture}[scale=0.45, transform shape]
\begin{scope}
\clip (0,0)-- +(120:\radius + 2) arc (120:0:\radius + 2) -- cycle;
\draw[red,thick,fill=red,fill opacity=0.2] (0,0) circle (\radius + 0.75);
\draw[red,thick,fill=white] (0,0) circle (\radius - 0.75);
\end{scope}

\begin{scope}
\clip (0,0)-- +(120:\radius + 2) arc (120:180:\radius + 2) -- cycle;
\draw[red,thick,fill=red,fill opacity=0.2] (\fpeval{\radius*cos(120*pi/180)},\fpeval{\radius*sin(120*pi/180)}) circle(0.75);
\end{scope}

\begin{scope}
\clip (0,0)-- +(0:\radius + 2) arc (0:-90:\radius + 2) -- cycle;
\draw[red,thick,fill=red,fill opacity=0.2] (\fpeval{\radius*cos(0*pi/180)},\fpeval{\radius*sin(0*pi/180)}) circle(0.75);
\end{scope}
\draw[blue,thick,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(240*pi/180)},\fpeval{\radius*sin(240*pi/180)}) circle(0.75);
\begin{scope}
\clip (0,0)-- +(0:\radius + 2) arc (0:-120:\radius + 2) -- cycle;
\draw[red,thick,dashed,fill=red,fill opacity=0.2] (0,0) circle (\radius + 0.9);
\draw[red,thick,dashed,fill=white] (0,0) circle (\radius - 0.9);
\end{scope}

\begin{scope}
\clip (0,0)-- +(0:\radius + 2) arc (0:45:\radius + 2) -- cycle;
\draw[red,thick,dashed,fill=red,fill opacity=0.2] (\fpeval{\radius*cos(0*pi/180)},\fpeval{\radius*sin(0*pi/180)}) circle(0.9);
\end{scope}

\begin{scope}
\clip (0,0)-- +(-120:\radius + 2) arc (-120:-180:\radius + 2) -- cycle;
\draw[red,thick,dashed,fill=red,fill opacity=0.2] (\fpeval{\radius*cos(-120*pi/180)},\fpeval{\radius*sin(-120*pi/180)}) circle(0.9);
\end{scope}

\draw[blue,thick,dashed,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(120*pi/180)},\fpeval{\radius*sin(120*pi/180)}) circle(0.9);

\fill[fill = white] (0,0) circle (\radius - 0.91);
\foreach \n in {0,1,2}{
	\draw (\fpeval{\radius*cos(\n*2*pi/3)},\fpeval{\radius*sin(\n*2*pi/3)}) node[circle,draw]{$\mygamma/3$};
}

\node[red] at (\fpeval{(\radius+1.25)*cos(2*pi/8)},\fpeval{(\radius+1.25)*sin(2*pi/8)}) {\Huge$\NE{a}_1$};

\node[blue] at (\fpeval{(\radius+1.5)*cos(4*pi/3)},\fpeval{(\radius+1.5)*sin(4*pi/3)}) {\Huge$\opt{a}_1$};

\node[red] at (\fpeval{(\radius+1.5)*cos(-2*pi/8)},\fpeval{(\radius+1.5)*sin(-2*pi/8)}) {\Huge$\NE{a}_2$};

\node[blue] at (\fpeval{(\radius+1.5)*cos(2*pi/3)},\fpeval{(\radius+1.5)*sin(2*pi/3)}) {\Huge$\opt{a}_2$};
\end{tikzpicture}
}
\raisebox{-0.55\height}{
\begin{tikzpicture}[scale=0.45, transform shape]
\draw[blue,thick,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(240*pi/180)},\fpeval{\radius*sin(240*pi/180)}) circle(0.75);
\draw[blue,thick,dashed,fill=blue,fill opacity=0.2] (\fpeval{\radius*cos(120*pi/180)},\fpeval{\radius*sin(120*pi/180)}) circle(0.9);



\fill[fill = white] (0,0) circle (\radius - 0.91);

\foreach \n in {0,1,2}{
	\draw (\fpeval{\radius*cos(\n*2*pi/3)},\fpeval{\radius*sin(\n*2*pi/3)}) node[circle,draw]{$\mybeta/3$};
}

\node[blue] at (\fpeval{(\radius+1.5)*cos(4*pi/3)},\fpeval{(\radius+1.5)*sin(4*pi/3)}) {\Huge$\opt{a}_1$};

\node[blue] at (\fpeval{(\radius+1.5)*cos(2*pi/3)},\fpeval{(\radius+1.5)*sin(2*pi/3)}) {\Huge$\opt{a}_2$};
\end{tikzpicture}
}
\end{center}
\vspace*{-7mm}
\caption{Game construction used to lower bound the price of anarchy for quadratic congestion games with fixed tolls $\tau\ge 3$ (left) and $\tau< 3$ (right). On the left (resp. right), the available actions of two of the eight (resp. three) agents are shown.  The solid red shape contains the resources utilized by the first user in the action $\NE{a}_1$, while the solid blue shape contains the resources utilized by the first user in the action $\opt{a}_1$. User 2 has similar actions but rotated clockwise on each circle by one resource. Each of the remaining agents' actions are defined similarly by rotating about the apparent ``ring''.}
\label{fig:fixedgame_high}
\end{figure}

==> Tex final - to submit ArXiv/figures-tex/figurecase1.tex <==
\begin{figure}[h!]
\begin{center}
\begin{tikzpicture}[scale=1]
\draw[thick,->] (0,0) -- (3.5,0);
\draw[thick] (3.7,0) -- (3.7,0) node[anchor=north east]{$\u$};
\draw[thick,->] (0,0) -- (0,3.5); 
\draw[thick] (0,3.7) -- (0,3.7) node[anchor=north east]{$\v$};
\draw[dashed] (0,0.5) -- (2,2) ;
\draw[dashed] (2,0) -- (2,3.3) ;
\node[rotate = 38] at (1,1.5) {$\u=\v$};
\node at (1,0.4) {\small Region A};
\node at (1,2.5) {\small Region B};
\node at (2.75,2) {\small Region C};
\draw[thick] (0,0.1) -- (0,-0.1) node[anchor=north]{\footnotesize$1$};
\draw[thick] (0.5,0.1) -- (0.5,-0.1)node[anchor=north]{\footnotesize$2$};
\draw[thick] (2,0.1) -- (2,-0.1);
\draw[thick] (2,-0.1) -- (2,-0.1)node[anchor=north]{\footnotesize$\bar{n}/2$};
\node[thick] (a) at (1.25,-0.3) {$\dots$};
\draw[thick] (0.1,0) -- (-0.1,0)node[anchor=east]{\footnotesize$0$};
\draw[thick] (0.1,0.5) -- (-0.1,0.5)node[anchor=east]{\footnotesize$1$};
\node[thick] (a) at (-0.3,1.1) {$\vdots$};
\end{tikzpicture}
\end{center}
\caption{Regions A, B, and C utilized in proof for the case $\u+\v\le n$.}
\label{fig:figure1proof}
\end{figure}

==> Tex final - to submit ArXiv/parts-body/abstract.tex <==
\begin{abstract}
\vspace*{1mm}
\begin{center}
First version:  {\it November 2019}.\quad This version:  {\it March 2021.}
\end{center}
\vspace*{3.5mm}
{\bf Abstract.} How can we design mechanisms to promote efficient use of shared resources? Here, we answer this question in relation to the well-studied class of atomic congestion games, used to model a variety of problems, including traffic routing.
% 
Within this context, a methodology for designing tolling mechanisms that minimize the system inefficiency (price of anarchy) exploiting solely local information is so far missing in spite of the scientific interest. 
%
In this manuscript we resolve this problem through a tractable linear programming formulation that applies to and beyond polynomial congestion games. When specializing our approach to the polynomial case, we obtain tight values for the optimal price of anarchy and corresponding tolls, uncovering an unexpected link with load balancing games.
%
We also derive optimal tolling mechanisms that are constant with the congestion level, generalizing the results of \cite{caragiannis2010taxes} to polynomial congestion games and beyond.
% 
Finally, we apply our techniques to compute the efficiency of the marginal cost mechanism. Surprisingly, optimal tolling mechanism using only local information perform closely to existing mechanism that utilize global information \cite{BiloV19}, while the marginal cost mechanism, known to be optimal in the continuous-flow model, has lower efficiency than that encountered levying \emph{no} toll.
%
All results are tight for pure \mbox{Nash equilibria, and extend to coarse correlated equilibria.}
\end{abstract}

% make title page
\maketitle

==> Tex final - to submit ArXiv/parts-body/ack-biblio.tex <==
%\begin{acks}
%ACKnolwedge XYZ
%\end{acks}

%% BIBLIO
\bibliographystyle{ACM-Reference-Format}
\bibliography{references.bib}



==> Tex final - to submit ArXiv/parts-body/introductionv3.tex <==
\section{Introduction}
Modern society is based on large-scale systems often at the service of end-users, e.g., transportation and communication networks. As the performance of such systems heavily depends on the interaction between the users' individual behaviour and the underlying infrastructure (e.g., drivers on a road-traffic network), the operation of such systems requires interdisciplinary considerations at the confluence between economics, engineering, and computer science.

A common issue arising in these settings is the performance degradation incurred when the users' individual objectives are not aligned to the ``greater good''. A prime example of how users' behaviour degrades the performance is provided by road-traffic routing: when drivers choose routes that minimize their individual travel time, the aggregate congestion could be much higher compared to that of a centrally-imposed routing. A fruitful paradigm to tackle this issue is to employ appropriately designed tolling mechanisms, as widely acknowledged in the economic and computer science literature \cite{morrison1986survey,bergendorff1997congestion,laffont2009theory}. 

Pursuing a similar line of research, this paper focuses on the design of tolling mechanisms that maximize the system efficiency associated with self-interested decision making in atomic \emph{congestion games}, i.e., that minimize the resulting \emph{price of anarchy} \cite{koutsoupias1999worst}. Within this context, we develop a methodology to compute the most efficient \emph{local} tolling mechanism, i.e., the most efficient mechanism whose tolls levied on each resource depend only on the local properties of that resource. We do so for both the congestion-aware and congestion-independent settings, whereby tolls have or do not have access to the current congestion levels. A summary of our results, including a comparison with the literature, can be found in \cref{tab:naware_vs_nagnostic}. Perhaps surprisingly, optimal local tolls deliver a price of anarchy close to that of existing tolls designed using global information \cite{BiloV19}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Congestion games, local and global mechanisms}
Congestion games were introduced in 1973 by Rosenthal  \cite{rosenthal1973class}, and since then have found applications in diverse fields, such as energy markets \cite{paccagnan2018nash}, machine scheduling \cite{suri2007selfish}, wireless data networks \cite{tekin2012atomic}, sensor allocation \cite{marden2013distributed}, network design \cite{anshelevich2008price}, and many more. While our results can be applied to a variety of problems, we consider traffic routing as our prime application.

In a congestion game, we are given a set of users $N=\{1,\dots,n\}$, and a set of resources $\mc{E}$. Each user can choose a subset of the set of resources which she intends to use. We list all feasible choices for user $i\in N$ in the set $\mc{A}_i\subseteq 2^{\mc{E}}$. The cost for using each resource $e\in\mc{E}$ depends only on the total number of users concurrently selecting that resource, and is denoted with $\ell_e :\mb{N}\rightarrow \mb{R}_{\ge0}$. Once all users have made a choice $a_i\in\mc{A}_i$, each user incurs a cost obtained by summing the costs of all resources she selected.  Finally, the system cost represents the cost incurred by \emph{all} users
%
\begin{equation}
\SC(a)=\sum_{i\in N}\sum_{e\in a_i} \ell_e(|a|_e),
\label{eq:systemcost}
\end{equation}
%
where $|a|_e$ is the number of users selecting resource $e$ in allocation $a=(a_1,\dots,a_n)$. We denote with $\mc{G}$ the set containing all congestion games with a maximum of $n$ agents, and where all resource costs $\{\ell_e\}_{e\in\mc{E}}$ belong to a common set of functions $\mc{L}$.

\paragraph{Local and global tolling mechanisms}
We assume users to be self-interested, and observe that self-interested decision making often results in a highly suboptimal system cost \cite{pigou}. Consequently,  there has been considerable interest in the application of tolling mechanisms to influence the resulting outcome \cite{morrison1986survey,bergendorff1997congestion,hearn1998solving,cole2006much,caragiannis2010taxes,BiloV19}. Formally, a tolling mechanism $T:G\times e\mapsto \tau_e$ is a map that associates an instance $G\in\mc{G}$ and a resource $e\in\mc{E}$ to the corresponding toll $\tau_e$. Here $\tau_e:\{1,\dots,n\}\rightarrow \mb{R}$ is a congestion-dependent toll, i.e., $\tau_e$ maps the number of users in resource $e$ to the corresponding toll. As a result, user $i\in N$ incurs a cost factoring both the cost of the resources and the tolls, i.e.,
%
\be
\C_i(a)=\sum_{e\in a_i} [\ell_e(|a|_e)+\tau_e(|a|_e)].
\label{eq:Ci}
\ee
%
Designing tolling mechanisms that utilize global information (such as knowledge of all resource costs, or knowledge of the feasible sets $\{\mc{A}_i\}_{i=1}^n$) is often difficult, as that might require the central planner to access private users information, in addition to the associated computational burden. Within the context of traffic routing (see \cref{ex:trafficroute} below), a global mechanism might produce a toll on edge $e$ that depends on the structure of the network, on the travel time over all edges, as well as on the exact origin and destination of every user. On the contrary, local tolling mechanisms require much less information, are scalable, accommodate resources that are dynamically added or removed, and are robust against a number of variations, e.g., the common scenario where drivers modify their destination. Therefore, a significant portion of the literature has focused on designing tolls that exploit only local information. Formally, we say that a tolling mechanism $T$ is \emph{local} if the toll on each resource only uses information on the cost function $\ell_e$ of the same resource $e$, and no other information.  If this is the case, we write $\tau_e = T(\ell_e)$ with slight abuse of notation. On the contrary, if the mechanism utilizes additional information on the instance, we say it is \emph{global}.

\begin{example}[traffic routing]
\label{ex:trafficroute}
Within the context of traffic routing, $\mc{E}$ represents the set of edges defining the underlying road network over which users wish to travel.
For this purpose, each user $i\in N$ can select any path connecting her origin to her destination node, thus producing a list of feasible paths $\mc{A}_i$. 
The travel time incurred by a user transiting on edge $e\in\mc{E}$ is captured by the function $\ell_e$, and depends only on the number of users traveling through that very edge. In this context, the function $\ell_e$ takes into consideration geometric properties of the edge, such as its length, the number of lanes and speed limit \cite{wardrop1952road}. The system cost in \eqref{eq:systemcost} represents the time spent on the network by \emph{all} users, whereas tolls are imposed on the edges to incentivize users in selecting paths \mbox{that minimize the total travel time \eqref{eq:systemcost}.}\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Performance metrics}
The performance of a tolling mechanism is typically measured by the ratio between the system cost incurred at the worst-performing emergent allocation and the minimum system cost. As users are assumed to be self-interested, the emergent allocation is described by any of the following equilibrium notions: pure or mixed Nash equilibrium, correlated or coarse correlated equilibrium -- each being a superset of the previous \cite{roughgarden2015intrinsic}.\footnote{For a congestion game, existence of pure Nash equilibria (and thus of all other equilibrium notions mentioned above) is guaranteed even in the presence of tolls, due to the fact that the resulting game is potential.} When considering pure Nash equilibria, the performance of a mechanism $T$, referred to as the \emph{price of anarchy} \cite{koutsoupias1999worst}, is defined as
%
\begin{equation}
\poa(T) = \sup_{G\in\mc{G}} \frac{\PNEcost(G,T)}{\mincost(G)},
\label{eq:poadef}
\end{equation}
%
where $\mincost(G)$ is the minimum social cost for instance $G$ as defined in \eqref{eq:systemcost}, and $\PNEcost(G,T)$ denotes the highest social cost at a Nash equilibrium obtained when employing the mechanism $T$ on the game $G$. Similarly, it is possible to define the price of anarchy for mixed Nash, correlated and coarse correlated equilibria. While these different metrics need not be equal in general, they do \emph{coincide} within the setting of interest to this manuscript, as we will later clarify. Therefore, in the following, we will use $\poa(T)$ to refer to the efficiency values of any and all \mbox{these equilibrium classes.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Related work}
The interest in the design of tolls dates back to the early 1900s \cite{pigou}. Since then, a large body of literature in the areas of transportation, economics, and computer science has investigated this approach \cite{morrison1986survey,cole2006much,bergendorff1997congestion,hearn1998solving,sandholm2002evolutionary}. Designing tolling mechanisms that optimize the efficiency is particularly challenging in the context of (atomic) congestion games, as observed, e.g., by \cite{harks2019pricing}, in part due to the multiplicity of the equilibria. While most of the research \cite{awerbuch2005price,christodoulou2005price,aland2006exact, roughgarden2015intrinsic} has focused on providing efficiency bounds for given schemes or in the un-tolled case, much less is known regarding the \emph{design} question. Owing to the technical difficulties, only partial results are available for global tolling mechanisms \cite{caragiannis2010taxes, fotakis2008cost, BiloV19}, while results for local mechanisms are limited to affine \mbox{congestion games \cite{caragiannis2010taxes}.}

Reference \cite{caragiannis2010taxes} initiated the study of tolling mechanisms in the context of congestion games, restricting their attention to affine resource costs. Relative to this setting, they show how to compute a congestion-independent global toll yielding a (tight) price of anarchy of $2$ for mixed Nash equilibria, in addition to a congestion-independent local toll yielding a (tight) price of anarchy of $1+2/\sqrt{3}\approx 2.155$ for pure Nash equilibria. Our result pertaining to the design of optimal \emph{congestion-independent local} tolls generalizes this finding to any polynomial (and non polynomial) congestion game and holds tightly for both pure Nash and coarse correlated equilibria.

More recently \cite{BiloV19} studies congestion-dependent global tolls for pure Nash and coarse correlated equilibria, in addition to one-round walks from the empty state. Relative to unweighted congestion games, they derive tolling mechanisms yielding a price of anarchy for coarse correlated equilibria equal to $2$ for affine resource costs; and similarly for higher order polynomials. While the latter work provides a number of interesting insights (e.g., some closed form price of anarchy expressions), all the derived tolling schemes require global information such as network and user knowledge - an often impractical scenario. In contrast, our results on \emph{optimal local tolls} focuses on the design of optimal mechanisms that exploit local information only, and thus are more widely applicable. Even if utilizing much less information, optimal local mechanisms are still competitive. For example, congestion-dependent optimal local tolls yield a price of anarchy of $2.012$ for coarse correlated equilibria and affine congestion games (to be compared with a value of $2$ mentioned above).

Related works have also explored modifications of the setup considered here:  \cite{caragiannis2010taxes} also studies singleton congestion games, \cite{fotakis2008cost} focuses on symmetric network congestion games, \cite{milchtaich2020internalization} on altruistic congestion games, while \cite{HarksKKM15, HoeferOS08, JelinekKS14} consider tolling a subset of the resources. Preprint \cite{skopalik2020improving} focuses on the computation of approximate Nash equilibria in atomic congestion games. Therein, the authors design modified resource costs leveraging a methodology \mbox{similar to that developed in~\cite{chandan2019when, DBLP:conf/netecon/ChandanPFM19,paccagnan2019incentivizing}.}

Finally, we note that the design of tolling mechanisms is far better understood when the original congestion game is replaced by its continuous-flow approximation, as uniqueness of the Nash equilibrium is guaranteed. Limited to this setting, marginal cost tolls produce an equilibrium which is always optimal~\cite{Beckmann1956}. Within the atomic setting, our work demonstrates that marginal cost tolls do not improve - and instead significantly deteriorate - the resulting system efficiency.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preview of our contributions}
The core of our work is centred on designing optimal local tolling mechanisms and on deriving their corresponding prices of anarchy for various classes of congestion games. Our work develops on parallel directions, and the contributions include the following:
%
\begin{itemize}
	\item[i)] The design of optimal local tolling mechanisms;
	\item[ii)] The design of optimal congestion-independent local tolling mechanisms;
	\item[iii)] The study of marginal cost tolls and their inefficiency.
\end{itemize}
%
\cref{tab:naware_vs_nagnostic} highlights the impact of our results on congestion games with polynomial cost functions of varying degree, though our methodology extends further. The following paragraphs describe our contributions in further details, while supporting Python and Matlab code can be found in~\cite{Chandancode19}. 

\input{parts-body/table-optimal-poa.tex}

\paragraph{Optimal local tolls}
In \cref{thm:main-thm,thm:simplifiedLP-explicit-solution} we provide a methodology for computing optimal local tolling mechanisms for congestion games. The resulting price of anarchy values for the case of polynomial congestion games are presented in \cref{tab:naware_vs_nagnostic} (fourth column), where we provide a comparison with those derived in \cite{caragiannis2010taxes,BiloV19} (third column), which instead make use of global information, for example, by letting the tolling function on resource $e$ depend on \emph{all} the other resource costs. Perhaps unexpectedly, the efficiency of optimal tolls designed using only local information is almost identical to that of existing tolls designed using global information \cite{caragiannis2010taxes,BiloV19}. In addition to providing similar performances by means of less information, local tolls are robust against uncertain scenarios (e.g., modifications in the origin/destination pairs) and can be computed efficiently.

Extensive work has focused on quantifying the price of anarchy for load balancing games, that is congestion games where all action sets are singletons, i.e., $\mc{A}_i\subseteq\mc{E}$. Within this setting, and when all resource costs are affine and identical, the price of anarchy is $\approx2.012$ \cite{suri2007selfish, CaragiannisFKKM11}. Our results connect with this line of work, demonstrating that optimally tolled affine congestion games have a price of anarchy  matching this value, and are tight already within this class. Stated differently, the price of anarchy of un-tolled and optimally tolled affine load balancing games with identical resources is the same. We believe such statement holds true more generally.

\paragraph{Optimal congestion-independent local tolls}
Our methodology can also be exploited to derive optimal local mechanisms under more stringent structural constraints. One such constraint, studied in numerous settings, consists in the use of congestion-independent mechanisms, which are attractive because of their simplicity. A linear program to compute optimal congestion-independent local mechanisms is presented in \cref{thm:congestion-indep}, while the corresponding optimal prices of anarchy for the case of polynomial congestion games are displayed in \cref{tab:naware_vs_nagnostic} (fifth column) and derived in \cref{cor:constanttollsd=2} as well as \cref{sec:congestion-indep}. All the results are novel, except for the case of $d=1$, which recovers \cite{caragiannis2010taxes}. We observe that the performance of congestion-independent mechanisms is comparable with that of congestion-aware mechanisms for polynomials of low degree ($d\le 3$), and still a good improvement over the un-tolled setup for high degree polynomials. In these cases, congestion-independent mechanisms are not only robust and simple to implement, but also relatively efficient.

\paragraph{Marginal cost tolls are worse than no tolls}
In non-atomic congestion games, any Nash equilibrium resulting from the application of the marginal contribution mechanism is optimal, i.e., it has a price of anarchy equal to one. \cref{cor:marginalcost} shows how to utilize our approach to compute the efficiency of the marginal cost mechanism in the \emph{atomic} setup. The resulting values of the price of anarchy are presented in the last column of Table~\ref{tab:naware_vs_nagnostic} for polynomial congestion games. While the marginal cost mechanism ensures that a Nash equilibrium is optimal (i.e., its price of stability is one), utilizing the marginal cost mechanism on the atomic model yields a price of anarchy that is \emph{worse} than that experienced levying no toll at all (compare the second and last column in Table~\ref{tab:naware_vs_nagnostic}). In other words, the design principle derived from the continuous-flow model does not carry over to the original atomic setup. This phenomenon manifests itself already in very simple settings, as we demonstrate in \cref{example:tolledpigouvian}.
We conclude by observing that our result differs significantly from that in \cite{meir2016marginal}, where the authors show that, as the number of agents grow large, marginal cost tolls become optimal. This difference stems from the fact that, in \cite{meir2016marginal}, the network structure is \emph{fixed} as the number of agents grows, whereas the worst case instance in our setting is a function of the number of agents.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Techniques and high-level ideas}
Underlying the developments presented above are a number of technical results, which stem from the observation that, in the majority of the existing literature, the set $\mc{L}$ contains all resource costs of the form $\ell(x)=\sum_{j=1}^m\alpha_jb_j(x)$ with $\alpha_j\ge0$, and given basis functions $\{b_1, \dots,b_m\}$. This describes the fact that each resource cost featured in the corresponding game belongs to a known class of functions. For example, in polynomial congestion games of maximum degree $d$, each resource is associated to a cost of the form $\alpha_1+\alpha_2 x+\dots +\alpha_{d+1} x^d$, corresponding to the choice of basis functions $\{1,\dots,x^d\}$. More generally, the decomposition $\ell(x)=\sum_{j=1}^m\alpha_jb_j(x)$ allows us to leverage a common framework to study different classes of problems not limited to polynomial congestion~games.
  
  In this context, we first show in \cref{thm:main-thm} that an optimal local tolling mechanisms is a linear map from the set of resource costs to the set of tolls. More precisely, we show that, for every resource cost $\ell(x)=\sum_{j=1}^m \alpha_j b_j(x)$, there exists an optimal local mechanism satisfying $\opt{T}(\ell)=\opt{T}(\sum_{j=1}^m \alpha_jb_j)=\sum_{j=1}^m \alpha_j \opt{T}(b_j)$, where the mechanism is obtained as a linear combination of $\opt{T}(b_j)$, with the \emph{same} coefficients $\alpha_j$ used to define $\ell$.\footnote{As word of caution, we  remark that linearity of the optimal mechanism in the sense clarified above does \emph{not} mean that the corresponding tolls are linear in the congestion level, i.e., does \emph{not} mean that $\tau_e(x)=a_ex+b_e$ for some $a_e,b_e$.} It is worth noting that this first result allows for a decoupling argument, whereby an optimal tolling function $\opt{T}(b_j)$ can be  separately computed for each of the basis $b_j$. 
The key idea underpinning the result on linearity of optimal tolls lies in observing that any congestion game utilizing resource cost functions with coefficients $\alpha_j\in\mb{R}_{>0}$ and a possibly non-linear tolling mechanism $T$, can be mapped to a corresponding congestion game where i) all coefficients $\alpha_j$ are identical to one, ii) only the linear part of the tolling mechanism $T$ is used, and iii) the price of anarchy is identical to that of the original game (as the number of resources grows). 
Complementary to this, our second result in \cref{thm:main-thm} reduces the problem of designing optimal basis tolls $\{\opt{T}(b_j)\}_{j=1}^m$ to a polynomially solvable linear program that also returns the tight value of the optimal price of anarchy. We do so by building upon the results in \cite{chandan19optimaljournal, paccagnan2018distributed}, which allow us to determine the performance of a tolling mechanism through the solution of a linear program (see \cref{linprog:characterize_poa}), in a similar spirit to \cite{BiloV19}, although with a provably tight characterization for \emph{any} number of agents and tolling function. We exploit this result and construct a polynomially-sized linear program that, for a given basis $b_j$, \mbox{searches over all linear tolls to find~$\opt{T}(b_j)$.}

When the basis functions are convex and increasing (e.g., in the well-studied polynomial case), we are able to explicitly solve the linear program and provide an analytic expression for the optimal tolling function, as well as a semi-analytic expression for optimal price of anarchy (\cref{thm:simplifiedLP-explicit-solution}). The fundamental idea consists in showing that the set of active constraints at the solution gives rise to a telescopic recursion, whereby the optimal toll to be levied when $u+1$ agents are selecting a resource can be written as a function of the optimal toll to be levied when only $u$ agents are present. This is the most technical part of the manuscript, and the expression of the optimal price of anarchy reveals an unexpected connection with that for un-tolled load balancing games on identical machines \cite{suri2007selfish, CaragiannisFKKM11}.
While the sizes of the linear programs appearing in \cref{thm:main-thm,thm:simplifiedLP-explicit-solution} grow (polynomially) with the number of agents $n$, in \cref{sec:largen} we show how to design optimal tolling mechanisms that apply to any $n$ (possibly infinite). Our approach consists in two steps: we first solve a linear program of finite dimension, and then extend its solution to arbitrary $n$.

Congestion-independent optimal local mechanisms as well as the efficiency of the marginal cost mechanism can also be  computed through linear programs (\cref{{thm:congestion-indep}} and \cref{cor:marginalcost}). In the first case, admissible tolls basis $\{\opt{T}(b_j)\}_{j=1}^m$ are constrained to be constant with the congestion, while in the second case the expression for marginal cost tolls is substituted in the program. We provide analytical solutions to these two programs for the case of polynomial congestion games.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Organization}
In \cref{sec:optimal-tolls} we derive linear programs to compute optimal local tolling mechanisms. We also provide optimal price of anarchy values for polynomial congestion games. In \cref{sec:explicit-expression} we obtain an explicit solution to these programs that applies when resource costs are convex and increasing.
\cref{sec:largen} generalizes the previous results to arbitrarily large number of agents. In \cref{sec:congestion-indep} and \cref{sec:pigouvtolls} we derive congestion independent tolling mechanism and evaluate the efficiency of the marginal cost mechanism. In these sections we also specialize \mbox{the results to the polynomial case.}

==> Tex final - to submit ArXiv/parts-body/table-optimal-poa.tex <==
\begin{table}[t!]%
\centering%
    \begin{tabular}{S[table-format=1]||S[table-format=5.3]|S[table-format=3]|S[table-format=3.3]|S[table-format=4.3]|S[table-format=2.2]}%
    {$d$}&{No toll}&{Global toll}&{Optimal local toll}&{Optimal constant local toll}&{Marginal cost toll}\\
        &{\cite{aland2006exact}}&{from \cite{caragiannis2010taxes,BiloV19}}&  {(this work)}&{(this work)}&{(this work)}\\
        \hline%
        1 & 2.50 & 2 & 2.012 &  2.15
        &3.00\\
        2 & 9.58 &  5 & 5.101 & 5.33 &13.00\\
        3 & 41.54 & 15 & 15.551 &  18.36 &57.36\\
        4 & 267.64 & 52 & 55.452 &  89.41 &391.00\\
        5 & 1513.57 & 203 & 220.401 &  469.74 &2124.21\\
        6 & 12345.20 & 877 & 967.533 &  3325.58 &21337.00\\
    \end{tabular}%
\vspace*{0.5mm}
    \caption{Price of anarchy values for congestion games with resource costs of degree at most $d$. All results are tight for pure Nash and also hold for coarse correlated equilibria. 
    The columns feature the price of anarchy with no tolls, with global tolls from \cite{caragiannis2010taxes,BiloV19}, with optimal local tolls, with optimal constant (i.e. congestion-independent) local tolls, and with marginal cost tolls, respectively. Columns four, five, and six, are composed of entirely novel results, except for the case of constant tolls with $d=1$, which recovers \cite{caragiannis2010taxes}. Note that i) optimal tolls relying only on local information perform closely to optimal tolls designed using global information, with a difference in performance below $1\%$ for $d=1$; ii) congestion-independent tolls result in a price of anarchy that is comparable to that obtained using congestion-aware local tolls for polynomials of low degree. The code used to generate this table can be downloaded from~\cite{Chandancode19}.}%
\label{tab:naware_vs_nagnostic}%
\vspace*{-7.5mm}
\end{table}

==> Tex final - to submit ArXiv/parts-body/table-ub-lb.tex <==
\begin{table}[t!]%
\centering%
    \begin{tabular}{S[table-format=2]||S[table-format=2.6]|S[table-format=1.7]|S[table-format=2.6]|S[table-format=1.7]|S[table-format=3.6]|S[table-format=2.7]}%
    \multicolumn{1}{c||}{$\bar n$} & \multicolumn{2}{c|}{$d=1$} & \multicolumn{2}{c|}{$d=2$} & \multicolumn{2}{c}{$d=3$}\\
    &{LB}&{UB}& {LB}&{UB}& {LB}&{UB} \\
        \hline
        10 & 2.011825 & 2.038237 & 5.097187 & 5.316382 &15.530175 & 17.138429\\
        20 & 2.012067 & 2.019844 & 5.100974 & 5.147543 &15.550847 & 15.751993\\
        30 & 2.012067 & 2.014335 & 5.100974 & 5.119149 &15.550852 & 15.684195 \\
        40 & 2.012067 & 2.012067 & 5.100974 & 5.100974 &15.550852 & 15.550859\\
    \end{tabular}

\vspace*{1mm}
    \caption{Lower and upper bounds (LB and UB) on the values of the optimal price of anarchy for polynomial congestion games with arbitrarily large number of agents and $d=1,2,3$. The LB vs UB shows how the tolls derived from $\myf$ defined in  \eqref{eq:definefext} are approximately optimal up the fifth decimal digit when we select $\bar n=40$.}%
\label{tab:ub-lb}%
\vspace*{-8mm}
    \end{table}

==> Tex final - to submit ArXiv/parts-frontmatter/frontmatter.tex <==
%% \BibTeX command to typeset BibTeX logo in the docs
%\AtBeginDocument{%
%  \providecommand\BibTeX{{%
%    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

% Replace when complete the rights form.
%\setcopyright{acmcopyright}
%\copyrightyear{2018}
%\acmYear{2018}
%\acmDOI{10.1145/1122445.1122456}


%% These commands are for a JOURNAL article.
\acmJournal{TEAC}
%\acmVolume{37}
%\acmNumber{4}
%\acmArticle{111}
%\acmMonth{8}


\title{Optimal Taxes in Atomic Congestion Games}
%
\author{Dario Paccagnan}
   \affiliation{%
   \institution{Imperial College London}   
   \department{Department of Computing}
   \city{London}
   \country{UK}
   }
\email{d.paccagnan@imperial.ac.uk}
%
\author{Rahul Chandan}
\affiliation{%
   \institution{University of California at Santa Barbara}   
   \department{Center for Control, Dynamical Systems and Computation}
   \city{Santa Barbara}
   \state{CA}
   \postcode{93105}
   \country{USA}
   }
\email{rchandan@ucsb.edu}
%
\author{Bryce L. Ferguson}
\affiliation{%
   \institution{University of California at Santa Barbara}   
   \department{Center for Control, Dynamical Systems and Computation}
   \city{Santa Barbara}
   \state{CA}
   \postcode{93105}
   \country{USA}
}
\email{blf@ucsb.edu}
%
\author{Jason R. Marden}
\affiliation{%
   \institution{University of California at Santa Barbara}   
   \department{Center for Control, Dynamical Systems and Computation}
   \city{Santa Barbara}
   \state{CA}
   \postcode{93105}
   \country{USA}
}
\email{jrmarden@ucsb.edu}
% concise list of authors' names for header
\renewcommand{\shortauthors}{Paccagnan, et al.}


%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003752</concept_id>
<concept_desc>Theory of computation</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003752.10010070.10010099.10010100</concept_id>
<concept_desc>Theory of computation~Algorithmic game theory</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003752.10010070.10010099.10010104</concept_id>
<concept_desc>Theory of computation~Quality of equilibria</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003752.10010070.10010099.10010109</concept_id>
<concept_desc>Theory of computation~Network games</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Theory of computation}
\ccsdesc[500]{Theory of computation~Algorithmic game theory}
\ccsdesc[500]{Theory of computation~Quality of equilibria}
%\ccsdesc[500]{Theory of computation~Network games}


\keywords{
Congestion games, 
optimal taxation mechanisms,
price of anarchy, 
Nash equilibrium,
coarse correlated equilibrium,
selfish routing, 
approximation algorithms.
}

\thanks{This manuscript has been deposited to the arXiv on 22 Nov 2019. A preliminary version appeared in ``Proceedings of the 14th Workshop on the Economics of Networks, Systems and Computation'' (NetEcon '19), see \cite{DBLP:conf/netecon/ChandanPFM19}. This research was carried out when the first author was affiliated with the University of California at Santa Barbara. This work was supported by the Swiss National Science Foundation Grant P2EZP2\_181618, ONR Grant \#N00014-20-1-2359, AFOSR Grant \#FA9550-20-1-0054.
}


==> Tex final - to submit ArXiv/parts-frontmatter/packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts} 
\usepackage{bbm}
\usepackage{xcolor}
\usepackage{pgfplots} 
\usepackage{graphicx} 
\usepackage{xfrac}
\usepackage{tikz}
\usepackage{hyperref}
\usepackage[capitalise]{cleveref}
\usepackage[font=small, tablename=Table]{caption}
\usepackage{subcaption}
\usepackage{tcolorbox}
\usepackage{tikz-network}
\usepackage{textpos}
\usepackage{xfp}
\usepackage{pgffor}
\usepackage{siunitx}
\usepackage{multirow}
\usepackage{wrapfig}
\usepackage{enumitem}
\usepackage[short,nocomma]{optidef}


\newtheorem{claim}{Claim}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem_mainresult}{Optimal Tolls}%
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}

\newtheorem*{sassumption}{Standing Assumption}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\poa}{\mathrm{PoA}}
\newcommand{\bu}{\bar{u}}
\newcommand{\npoa}{\mathrm{NPoA}}
\newcommand{\cg}{\mathcal{G}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}	
\newcommand{\actionset}{\mathcal{A}}
\newcommand{\latencyset}{\mathcal{L}}
\newcommand{\taxmechanism}{T}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbb{#1}}
\newcommand{\resset}{\mc{E}}
\newcommand{\DP}[1]{{\color{red} {#1}}}
\newcommand{\IR}{\mathcal{I}}
\newcommand{\eqcost}{{\tt{EqCost}}}
\newcommand{\PNEcost}{{\tt{NECost}}}
\newcommand{\PNEcostNR}{{\tt{NPNECost}}}
\newcommand{\CCEcost}{{\tt{CCECost}}}
\newcommand{\mincost}{{\tt{MinCost}}}
\newcommand{\SC}{{\rm{SC}}}
\renewcommand{\C}{{\rm{C}}}
\newcommand{\opt}[1]{{#1}^{\rm opt}}
\newcommand{\NE}[1]{{#1}^{\rm ne}}
\newcommand{\pig}[1]{{#1}^{\rm p}}
\pgfplotsset{compat=1.15}
\newcommand{\myf}{f^{\infty}}
\newcommand{\Thathat}{\bar{T}}
\newcommand{\SM}{Supplementary Information}
\renewcommand{\u}{u}
\renewcommand{\v}{v}
\newlength{\mynegspace}
\setlength{\mynegspace}{-0.6mm}
\newcommand{\mybeta}{c_2}
\newcommand{\mygamma}{c_1}
\newcommand{\mynu}{\lambda}
\newcommand{\nquad}{\mkern-15mu}

\newcommand{\jRC}{u}
\newcommand{\ellRC}{v}

\renewcommand{\star}{\ast}
\newcommand{\q}{q}

\usetikzlibrary{shapes.misc}
\tikzset{cross/.style={cross out, draw, 
         minimum size=2*(#1-\pgflinewidth), 
         inner sep=0pt, outer sep=0pt}}
         
\usepackage{xr}
\definecolor{pnasblueback}{RGB}{205,217,235}

%\newcommand\DPmargin[1]{\marginpar{\color{red} \tiny\ttfamily #1}}
